Fock-Goncharov conjecture and polyhedral cones for $U \subset SL_n$ and base affine space $SL_n /U$

I prove several conjectures of \cite{GHKK} on the cluster structure of $SL_n$, which in particular imply the full Fock-Goncharov conjecture for the open double Bruhat cell $\mathcal{A} \subset SL_n/U$, for $U \subset SL_n$ a maximal unipotent subgroup. This endows the mirror cluster variety $\mathcal{X}$ with a canonical potential function $W$, and determines a canonical cone $W^T \geq 0 \subset \mathcal{X}\left(\mathbb{R}^T\right)$ of the mirror tropical space, whose integer points parametrize a basis of $H^0\left(SL_n/U,\mathcal{O}_{SL_n/U}\right)$, canonically determined by the open subset $\mathcal{A} \subset SL_n/U$. Each choice of seed identifies $\mathcal{X}\left(\mathbb{R}^T\right)$ with a real vector space, and $W^T \geq 0$ with a system of linear equations with integer coefficients, cutting out a polyhedral cone. We obtain in this way (generally) infinitely many parameterizations of the canonical basis as integer points of a polyhedral cone. For the usual initial seed of the double Bruhat cell, we recover the parametrizations of Berenstein-Kazhdan\cite{BKaz,BKaz2} and Berenstein-Zelevinsky\cite{BZ96} by integer points of the Gelfand-Tsetlin cone.

==> Qs0n3.tex <==
% U quiver
%\begin{minipage}{\linewidth}% to keep image and caption on one page
\begin{center}
\begin{tikzpicture}
	\node (13) at (4,0) [draw, regular polygon, regular polygon sides=4, inner sep=0pt] {$v_{1;3}$};
	\node (12) at (6,0) {$v_{1;2}$};

	\node (23) at (5,1) [draw, regular polygon, regular polygon sides=4, inner sep=0pt] {$v_{2;3}$};


% horizontal
	\draw[->] (13) -- (12) ;

% up left
	\draw[->] (12) -- (23) ;
\end{tikzpicture}.
%\captionof{figure}{Quiver for $\mathring{U} \subset SL_5 $ and $\vb{i}_{w_0} = 1,2,1,3,2,1,4,3,2,1$ \label{fig:U_quiver}}
\end{center}
%\end{minipage}



==> Qspn3.tex <==
% U quiver
%\begin{minipage}{\linewidth}% to keep image and caption on one page
\begin{center}
\begin{tikzpicture}
	\node (13) at (4,0) [draw, regular polygon, regular polygon sides=4, inner sep=0pt] {$v_{1;3}$};
	\node (12) at (6,0) {$v_{1;2}$};

	\node (23) at (5,1) [draw, regular polygon, regular polygon sides=4, inner sep=0pt] {$v_{2;3}$};


% horizontal
	\draw[<-] (13) -- (12) ;

% up left
	\draw[<-] (12) -- (23) ;
\end{tikzpicture},
%\captionof{figure}{Quiver for $\mathring{U} \subset SL_5 $ and $\vb{i}_{w_0} = 1,2,1,3,2,1,4,3,2,1$ \label{fig:U_quiver}}
\end{center}
%\end{minipage}



